Distribution of Faint Atomic Gas in Hickson Compact Groups

We present 21cm HI observations of four Hickson Compact Groups with evidence for a substantial intragroup medium using the Robert C. Byrd Green Bank Telescope (GBT). By mapping H I emission in a region of 25$^{\prime}\times$25$^{\prime}$ (140-650 kpc) surrounding each HCG, these observations provide better estimates of HI masses. In particular, we detected 65% more \HI than that detected in the Karl G. Jansky Very Large Array (VLA) imaging of HCG92. We also identify if the diffuse gas has the same spatial distribution as the high-surface brightness (HSB) HI features detected in the VLA maps of these groups by comparing the HI strengths between the observed and modeled masses based on VLA maps. We found that the HI observed with the GBT to have a similar spatial distribution as the HSB structures in HCGs 31 and 68. Conversely, the observed HI distributions in HCGs44 and 92 were extended and showed significant offsets from the modeled masses. Most of the faint gas in HCG44 lies to the Northeast-Southwest region and in HCG 92 lies in the Northwest region of their respective groups. The spatial and dynamical similarities between the total (faint+HSB) and the HSB HI indicate that the faint gas is of tidal origin. We found that the gas will survive ionization by the cosmic UV background and the escaping ionizing photons from the star forming regions and stay primarily neutral for at least 500 Myrs.

==> table_h1_mass.tex <==
\begin{deluxetable}{| l |c |c |c |c|c|}
\tablenum{3}
\tabletypesize{\scriptsize}
\tablecaption{HI masses for each pointing.  \label{tbl-hi_mass}}
\tablewidth{0pt}
\tablehead{
\colhead{} &  \colhead{HCG~31} & \colhead{HCG~44} & \colhead{HCG~68} & \colhead{HCG~92} }
\startdata
      11   &  <8.84  & 9.12  & 8.44  & <9.32
      12   &  9.04  & 9.16  & <8.45  & <9.32
      13   &  9.47  & 8.78  & <8.45  & <9.29
      14   &  9.42  & <8.41  & <8.41  & <9.28
      15   &  9.10  & <8.42  & <8.40  & <9.28
      21   &  9.25  & <8.43  & <8.39  & 9.64
      22   &  9.90  & 8.99  & <8.40  & 9.68
      23   &  10.11  & 9.23  & 9.08  & 9.77
      24   &  9.83  & 9.39  & 9.40  & <9.27
      25   &  8.90  & 9.03  & 9.13  & <9.27
      31   &  9.24  & 9.25  & 9.58  & <9.26
      32   &  10.04  & 9.51  & 9.80  & 9.59
      33   &  10.26  & 9.51  & 9.62  & 10.20
      34   &  10.01  & 9.31  & 9.09  & 10.30
      35   &  9.37  & 8.88  & <8.35  & 10.13
      41   &  8.88  & 8.77  & <8.35  & 9.84
      42   &  9.76  & 9.05  & 9.19  & 10.17
      43   &  10.01  & 9.40  & 9.75  & 10.18
      44   &  9.80  & 9.50  & 9.91  & 9.60
      45   &  9.02  & 9.24  & 9.64  & <9.27
      51   &  <8.63  & 8.79  & 9.25  & <9.28
      52   &  9.09  & 9.17  & 9.55  & <9.29
      53   &  9.29  & 9.11  & 9.37  & 9.66
      54   &  9.06  & -Inf.00  & 8.73  & 9.65
      55   &  <8.56  & -Inf.00  & <8.30  & <9.27
\enddata
\end{deluxetable}


==> table_rho_values.tex <==
\clearpage
\begin{landscape}
\begin{deluxetable}{|c|c|c| c|c |c |c |c| c|c |c |c |c| c|c |c |c |c| c|c |c |c |c| c|c |c |c |}
\tablenum{5}
\tabletypesize{\scriptsize}
\tablecaption{Distance Between the Pointings. \label{tbl-rho_values}}
\tablewidth{0pt}
\tablehead{
\colhead{}  & \colhead{A1}  & \colhead{A2}  & \colhead{A3}  & \colhead{A4}  & \colhead{A5}   & \colhead{B1}  & \colhead{B2}  & \colhead{B3}  & \colhead{B4}  & \colhead{B5}   & \colhead{C1}  & \colhead{C2}  & \colhead{C3}  & \colhead{C4}  & \colhead{C5}   & \colhead{D1}  & \colhead{D2}  & \colhead{D3}  & \colhead{D4}  & \colhead{D5} & \colhead{E1}  & \colhead{E2}  & \colhead{E3}  & \colhead{E4}  & \colhead{E5}      }
\startdata
     
      E5 & 22.6 & 20.0 & 17.9 & 16.5 &16.0&  20.0 & 17.0 &14.4 & 12.6 & 12.0 & 19.7& 14.4 & 11.3 & 8.9 & 8.0 &  16.5 & 12.6 & 8.9 & 5.7 & 4.0  & 16.0 & 12.0 & 8.0 & 4.0 & 0.0     \\
     \hline
     E4 &  20.0 & 17.9 & 16.5 &16.0& 16.5& 17.0 &14.4 & 12.6 & 12.0 & 12.6  & 14.4 & 11.3 &8.9 & 8.0 & 8.9 & 12.6 & 8.9 & 5.7 &  4.0 & 5.7  & 12.0 & 8.0 & 4.0 & 0.0     \\
     \hline     
     E3 & 17.9 & 16.5 &16.0& 16.5 & 17.9 & 14.4 & 12.6 & 12.0 & 12.6 & 14.4  & 11.3 & 8.9 & 8.0 & 8.9 & 11.3  &8.9 & 5.7 & 4.0 & 5.7 & 8.9 &  8.0 & 4.0 & 0.0     \\
     \hline
     E2 & 16.5 &16.0& 16.5 & 17.9 & 20.0 &   12.6 & 12.0 & 12.6 & 14.4 & 17.0  & 8.9 & 8.0 & 8.9 & 11.3 & 14.4 &  5.7 & 4.0 & 5.7 & 8.9 & 12.6 &  4.0 & 0.0     \\
     \hline
     E1&  16.0& 16.5 & 17.9 & 20.0 & 22.7 & 12.0 & 12.6 & 14.4 & 17.0 & 20.0  & 8.0 & 8.9 & 11.3 & 14.4 & 19.7 & 4.0 & 5.7 & 8.9 & 12.6 & 16.5  & 0.0       \\
      \hline
     
     D5 & 20.0 & 17.0 &14.4 & 12.6 & 12.0 & 19.7& 14.4 & 11.3 & 8.9 & 8.0 & 16.5 & 12.6 & 8.9 & 5.7 & 4.0 &  16.0 & 12.0 & 8.0 & 4.0 & 0.0     \\
     \hline
     D4 & 17.0 &14.4 & 12.6 & 12.0 & 12.6 & 14.4 & 11.3 & 8.9 & 8.0 & 8.9 & 12.6 & 8.9 & 5.7 & 4.0 & 5.7  & 12.0 & 8.0 & 4.0 & 0.0     \\
     \hline     
     D3 & 14.4 & 12.6 & 12.0 & 12.6 & 14.4 & 11.3 & 8.9 & 8.0 & 8.9 & 11.3 & 8.9 & 5.7 & 4.0 & 5.7 & 8.9  &  8.0 &  4.0 & 0.0    \\
     \hline
     D2 & 12.6 & 12.0 & 12.6 & 14.4 & 17.0 & 8.9 & 8.0 & 8.9 & 11.3 & 14.4 & 5.7 &  4.0 & 5.7 & 8.9 & 12.6  &  4.0 & 0.0    \\
     \hline
     D1&  12.0 & 12.6 & 14.4 & 17.0 & 20.0 & 8.0 & 8.9 & 11.3 & 14.4 & 19.7 &   4.0 & 5.7 & 8.9 & 12.6 & 16.5  & 0.0       \\
     \hline
     
     C5 & 19.7& 14.4 & 11.3 & 8.9 & 8.0 &  16.5 & 12.6 & 8.9 & 5.7 & 4.0 & 16.0 & 12.0 & 8.0 &  4.0 & 0.0    \\
     \hline
     C4 & 14.4 & 11.3 & 8.9 & 8.0 & 8.9  & 12.6 & 8.9 & 5.7 & 4.0 & 5.7 & 12.0 & 8.0 &  4.0 & 0.0    \\
     \hline
     C3 & 11.3 & 8.9 & 8.0 & 8.9 & 11.3 & 8.9 & 5.7 & 4.0 & 5.7 & 8.9 & 8.0 &  4.0 & 0.0    \\
     \hline
     C2 &  8.9 & 8.0 & 8.9 & 11.3 & 14.4 &  5.7 & 4.0  & 5.7 & 8.9 & 12.6 & 4.0&  0.0 \\
     \hline
     C1&  8.0 & 8.9 & 11.3 & 14.4 & 19.7 &  4.0 & 5.7 & 8.9 & 12.6 & 16.5  & 0.0       \\
     \hline
     
     B5 &  16.5 & 12.6 & 8.9 & 5.7 & 4.0 & 16.0 & 12.0 & 8.0 & 4.0 & 0.0     \\
     \hline
     B4 & 12.6 & 8.9 & 5.7 &  4.0 & 5.7 & 12.0 & 8.0 & 4.0 & 0.0     \\
     \hline
     B3 & 8.9 & 5.7 & 4.0 & 5.7 & 8.9 & 8.0 & 4.0 & 0.0     \\
     \hline
     B2 & 5.7 & 4.0 & 5.7 & 8.9 & 12.6 & 4.0 &0.0  \\
     \hline
     B1&  4.0 & 5.7 & 8.9 & 12.6 & 16.5  & 0.0       \\
     \hline
     
     A5 & 16.0 & 12.0 & 8.0 & 4.0 & 0.0     \\ 
     \hline      
     A4 & 12.0 &  8.0 & 4.0 & 0.0    \\ 
     \hline
     A3 & 8.0 & 4.0 & 0.0   \\
     \hline
     A2 & 4.0 &   0.0  \\
     \hline
     A1 & 0.0    
    
\enddata
\end{deluxetable}

\clearpage 
\end{landscape}
